CPAchecker: A Tool for Configurable Software Verification

Configurable software verification is a recent concept for expressing different program analysis and model checking approaches in one single formalism. This paper presents CPAchecker, a tool and framework that aims at easy integration of new verification components. Every abstract domain, together with the corresponding operations, is required to implement the interface of configurable program analysis (CPA). The main algorithm is configurable to perform a reachability analysis on arbitrary combinations of existing CPAs. The major design goal during the development was to provide a framework for developers that is flexible and easy to extend. We hope that researchers find it convenient and productive to implement new verification ideas and algorithms using this platform and that it advances the field by making it easier to perform practical experiments. The tool is implemented in Java and runs as command-line tool or as Eclipse plug-in. We evaluate the efficiency of our tool on benchmarks from the software model checker BLAST. The first released version of CPAchecker implements CPAs for predicate abstraction, octagon, and explicit-value domains. Binaries and the source code of CPAchecker are publicly available as free software.

==> Makefile <==
# Makefile for papers
LATEX = pdflatex

# Run once, then re-run until it's happy
# Input redirected from /dev/null is like hitting ^C at first error
all:
	@echo $(LATEX) main.tex </dev/null
	@if $(LATEX) main.tex </dev/null; then \
		true; \
	else \
		stat=$$?; touch main.dvi; exit $$stat; \
	fi 
	#bibtex main
	@echo $(LATEX) main.tex </dev/null
	@while grep "Rerun to get cross" main.log; do \
		echo $(LATEX) main.tex </dev/null; \
		if $(LATEX) main.tex </dev/null; then \
			true; \
		else \
			stat=$$?; touch main.dvi; exit $$stat; \
		fi; \
	done
	@if grep "miktex" main.log ; then \
		cygstart main.pdf; \
	fi

clean:
	rm -f main.aux main.log main.out main.ps main.pdf main.dvi main.blg *.bak *.auto

